Information-Based Trajectory Planning for Spacecraft-to-Spacecraft Tracking and Navigation in Cislunar Space

We present a trajectory planning method that balances information collection and control effort to improve cislunar spacecraft-to-spacecraft absolute tracking. Expanding use of cislunar space requires alternative navigation and tracking procedures that minimize reliance on ground-based support. Among efforts to address this need, spacecraft-to-spacecraft tracking exploits nonlinear dynamical tracers encoded in a series of relative measurements to infer absolute states of both an observer and a target. The geometry between spacecraft operating under this mode can significantly influence tracking performance. This work considers this geometrical impact by designing observer trajectories that jointly balance control effort and an information-theoretic quantification of the expected spacecraft-to-spacecraft tracking performance. Our methods are designed for multiple low-thrust observation platforms of various sensing modalities and can incorporate multiple space object targets in planning. By leveraging information gain in the optimal control problem, we report almost an order of magnitude improvement in the expected navigation and tracking errors for an optical observer operating in a Distant Retrograde Orbit (DRO). This work demonstrates the feasibility and value of information-optimal low-thrust spacecraft trajectory design for current and upcoming cislunar missions.

==> Old/Outline.tex <==



What are the sections that I want? 

\begin{itemize}
    \item Introduction 
    %
    \item Information Collection \begin{itemize}
        \item Begin by establishing the two filtering cases that we are considering 
        \item One includes the case where we assume we know the state of the observer 
        \item The other assumes that we do not know the state of the observer 
        \item We assume any measurement modality 
        \item Look at Greaves and Psiaki papers to understand how to formulate this section 
        \item You need to think carefully about how to structure this so that it is not too much information for the reader to digest
    \end{itemize}
    %
    \item Information Gain and the KL divergence 
    \begin{itemize}
        \item Introduce first as a general form of two pdfs 
        \item Then, impose the Gaussian assumptions 
        \item Then, introduce the first and second order forms 
        \item \textcolor{red}{Should some of the derivations be included as an appendix?}
        \item \textcolor{red}{What about the partials, should these be included as an appendix}
        \item Show examples comparing the first and second order moment approximations in for different measurement modalities \begin{itemize}
            \item What should I do for this?
            \item NRHO \textit{and} DRO?
            \item Different uncertainty levels?
            \item Different measurement modalities 
            \item How to convey to the reader the dependence on separation? 
        \end{itemize}
    \end{itemize}
    

    
    \item Information-Based Optimal Control \begin{itemize}
        \item 
    \end{itemize} 
    \item Successive Convex Programming \begin{itemize}
        \item 
    \end{itemize} 
    \item Numerical Test Cases \begin{itemize}
        \item 
    \end{itemize} 
    %
\end{itemize}

==> Old/information_objective.tex <==
%
Define an initial \textit{augmented} state that concatenates the state of the sensor and the states of the catalog targets
%
\begin{equation}
    \boldsymbol{x}_{{\textstyle\mathstrut}A, 0} \sim \mathcal{N}\left(\bar{\boldsymbol{x}}_{{\textstyle\mathstrut}A, 0}, P_{{\textstyle\mathstrut}A, 0} \right)
\end{equation}
%
where,
%
\begin{equation}
    \bar{\boldsymbol{x}}_{{\textstyle\mathstrut}A, 0} = \left[ \bar{\boldsymbol{x}}_{{\textstyle\mathstrut}S, 0}^\top, \bar{\boldsymbol{x}}_{{\textstyle\mathstrut}T_1, 0}^{\top}, \cdots,  \bar{\boldsymbol{x}}_{{\textstyle\mathstrut}T_{N_{T}}, 0}^{\top} \right]^\top,
\end{equation}
%
and, 
%
\begin{equation}
    P_{{\textstyle\mathstrut}A, 0} = \text{diag}\left( P_{{\textstyle\mathstrut}S, 0}, P_{{\textstyle\mathstrut}T_1, 0}, \cdots, P_{{\textstyle\mathstrut}T_{N_T}, 0} \right)
\end{equation}


\begin{equation}
    \boldsymbol{x}_{{\textstyle\mathstrut}T_i, \ell + 1} = \boldsymbol{f}_\ell\left(\boldsymbol{x}_{{\textstyle\mathstrut}T_i, \ell}\right) + \boldsymbol{v}_{{\textstyle\mathstrut}T_i, \ell}\mbox{,}\hspace{0.25cm} \text{for } i = {1, 2, \cdots, N_T},\label{eqn:target_dynamics_evolution}
\end{equation}
%
and,
%
\begin{equation}
    \boldsymbol{x}_{{\textstyle\mathstrut}S, \ell + 1} = \boldsymbol{f}_\ell\left(\boldsymbol{x}_{{\textstyle\mathstrut}S, \ell}\right) + \boldsymbol{v}_{{\textstyle\mathstrut}S, \ell},
\end{equation}
%
Additionally, for $\ell \in 1:N_{meas}$
%
\begin{equation}
    \boldsymbol{v}_{{\textstyle\mathstrut}A, \ell} = \left[ \boldsymbol{v}_{{\textstyle\mathstrut}S, \ell}^\top, \boldsymbol{v}_{{\textstyle\mathstrut}T_1, \ell}^{\top}, \cdots,  \boldsymbol{v}_{{\textstyle\mathstrut}T_{N_T}, \ell}^{\top} \right]^\top,
\end{equation}
%
Augmented discrete time transition 
%
\begin{equation}
    \boldsymbol{x}_{{\textstyle\mathstrut}A, \ell + 1} = \boldsymbol{f}_\ell\left(\boldsymbol{x}_{{\textstyle\mathstrut}A, \ell}\right) + \boldsymbol{v}_{{\textstyle\mathstrut}A, \ell}
\end{equation}
%
then 
%
\begin{equation}
    %
    \boldsymbol{X}_A = \boldsymbol{\mathcal{F}}\left( \boldsymbol{\Xi}_{A} \right) = 
    \begin{bmatrix}
        %
        \boldsymbol{x}_{A, 0}\\
        %
        \boldsymbol{f}_1\left(\boldsymbol{x}_{{\textstyle\mathstrut}A, 0}\right) + \boldsymbol{v}_{{\textstyle\mathstrut}A, 0}\\
        %
        \boldsymbol{f}_2\left(\boldsymbol{x}_{{\textstyle\mathstrut}A, 1}\right) + \boldsymbol{v}_{{\textstyle\mathstrut}A, 1}\\
        %
        \vdots\\
        %
        \boldsymbol{f}_{N_\text{meas}}\left(\boldsymbol{x}_{{\textstyle\mathstrut}A, N_\text{meas} - 1}\right) + \boldsymbol{v}_{{\textstyle\mathstrut}A, N_{\text{meas}} - 1}
    \end{bmatrix}
    %
\end{equation}
%
where
%
\begin{equation}
    \boldsymbol{\Xi}_{A} = \left[ \boldsymbol{x}_{{\textstyle\mathstrut}A, 0}^\top, 
    \boldsymbol{v}_{{\textstyle\mathstrut}A, 0}^{\top}, \cdots,  \boldsymbol{v}_{{\textstyle\mathstrut}A, N_{meas} - 1}^{\top} \right]^\top,
\end{equation}
%
Similarly, we can define an augmented measurement vector as 
%
\begin{equation}
    %
    \boldsymbol{Y}_A = \boldsymbol{\mathcal{H}}\left( \boldsymbol{\Xi}_{A} \right) = 
    \begin{bmatrix}
        %
        \boldsymbol{h}\left(\boldsymbol{x}_{ {\textstyle\mathstrut} A, 0}\right) + \boldsymbol{w}\\
        %
        \boldsymbol{h}\left(\boldsymbol{x}_{{\textstyle\mathstrut}A, 1}\right) + \boldsymbol{w}\\
        %
        \vdots\\
        %
        \boldsymbol{h}\left(\boldsymbol{x}_{{\textstyle\mathstrut}A, N_\text{meas} - 1}\right) + \boldsymbol{w}
    \end{bmatrix}
    %
\end{equation}
%
Then, let 
%
\begin{equation}
    \boldsymbol{Z}_A = \begin{bmatrix}
        \boldsymbol{X}_A\\
        \boldsymbol{Y}_A
    \end{bmatrix} =
    %
    \begin{bmatrix}
        \boldsymbol{\mathcal{F}}(\boldsymbol{\Xi}_A) \\
        \boldsymbol{\mathcal{H}}(\boldsymbol{\Xi}_A)
    \end{bmatrix} = 
    %
    \boldsymbol{\mathcal{G}}(\boldsymbol{\Xi}_A)
    %
\end{equation}

Second order Taylor series 

\begin{equation}
    \boldsymbol{Z}_A \simeq \bar{\boldsymbol{Z}}_A + \boldsymbol{\mathcal{G}}'\boldsymbol{e}_A + \boldsymbol{b}_A
\end{equation}

\begin{equation}
    \boldsymbol{b}_A = \frac{1}{2} \begin{bmatrix}
        %
        \boldsymbol{e}_A^\top \boldsymbol{\mathcal{G}}_1''\boldsymbol{e}_A\\
        %
        \boldsymbol{e}_A^\top \boldsymbol{\mathcal{G}}_2''\boldsymbol{e}_A\\
        %
        \vdots\\
        %
        \boldsymbol{e}_A^\top \boldsymbol{\mathcal{G}}_M''\boldsymbol{e}_A
        %
    \end{bmatrix} =
    %
    \frac{1}{2}\begin{bmatrix}
        \text{tr}\left(\boldsymbol{\mathcal{G}}_1'' \boldsymbol{e}_A \boldsymbol{e}^\top_A\right)\\
        %
        \text{tr}\left(\boldsymbol{\mathcal{G}}_2'' \boldsymbol{e}_A \boldsymbol{e}^\top_A\right)\\
        %
        \vdots \\
        %
        \text{tr}\left(\boldsymbol{\mathcal{G}}_M'' \boldsymbol{e}_A \boldsymbol{e}^\top_A\right)
    \end{bmatrix}
    %
\end{equation}

%

\begin{equation}
    \boldsymbol{\mathcal{G}}' = \frac{\partial \boldsymbol{\mathcal{G}}}{\partial \boldsymbol{\Xi}_A}\bigg|_{\bar{\boldsymbol{\Xi}}_A}
\end{equation}

%

\begin{equation}
    \boldsymbol{\mathcal{G}}_i'' = \frac{\partial^2 \boldsymbol{\mathcal{G}}_i}{\partial \boldsymbol{\Xi}_A \partial \boldsymbol{\Xi}^\top_A}\bigg|_{\bar{\boldsymbol{\Xi}}_A}
\end{equation}

\begin{align}
    \mathlarger{\Sigma}_{ {\textstyle\mathstrut} \boldsymbol{Z}_A \boldsymbol{Z}_A} &= \mathbb{E}\left[ \left(\boldsymbol{Z}_A - \bar{\boldsymbol{Z}}_A \right) \left(\boldsymbol{Z}_A - \bar{\boldsymbol{Z}}_A \right)^\top \right] \\
    &= \mathbb{E} \left[ \boldsymbol{\mathcal{G}}' \boldsymbol{e}_A \boldsymbol{e}_A^\top \boldsymbol{\mathcal{G}}'^\top \right] + \mathbb{E}\left[ \boldsymbol{b}_{A} \boldsymbol{e}_A^\top \boldsymbol{\mathcal{G}}'^\top \right] + \mathbb{E}\left[\boldsymbol{\mathcal{G}}' \boldsymbol{e}_A \boldsymbol{b}_A^\top \right] + \mathbb{E}\left[\boldsymbol{b}_A \boldsymbol{b}_A^\top \right] \\
\end{align}


\textit{Lemma 1:} If $\boldsymbol{\xi}$ is a zero-mean Gaussian vector-valued random variable with covariance $\Sigma$, then 

\begin{equation}
    \mathbb{E}\left[\boldsymbol{\xi}~\text{tr}\left(A \boldsymbol{\xi} \boldsymbol{\xi}^\top \right)\right] = \boldsymbol{0}
\end{equation}
%
and 
%
\begin{align}
    %
    \mathbb{E}\left[ \text{tr}\left( 
    A \boldsymbol{\xi} \boldsymbol{\xi}^\top B \boldsymbol{\xi} \boldsymbol{\xi}^\top \right) \right] &= \mathbb{E}\left[\text{tr}\left(A \boldsymbol{\xi} \boldsymbol{\xi}^\top\right) \text{tr}\left(B \boldsymbol{\xi} \boldsymbol{\xi}^\top\right)\right] \nonumber \\
    %
    &= 2~\text{tr}\left(A \Sigma B \Sigma \right) + \text{tr}\left( A \Sigma \right) \text{tr}\left( B \Sigma \right)
    %
\end{align}

\begin{equation}
    \mathlarger{\Sigma}_{ {\textstyle\mathstrut} \boldsymbol{Z}_A \boldsymbol{Z}_A} = \boldsymbol{\mathcal{G}}' \mathlarger{\Sigma}_{ {\textstyle\mathstrut} \boldsymbol{\Xi}_A \boldsymbol{\Xi}_A} \boldsymbol{\mathcal{G}}'^\top  + \mathlarger{\mathcal{B}}_A
\end{equation}

\begin{equation}
    \mathlarger{\mathcal{B}}_{A_{i, j}} = 2~\text{tr}\left( \boldsymbol{\mathcal{G}}_i'' \mathlarger{\Sigma}_{ {\textstyle\mathstrut} \boldsymbol{\Xi}_A \boldsymbol{\Xi}_A} \boldsymbol{\mathcal{G}}_j'' \mathlarger{\Sigma}_{ {\textstyle\mathstrut} \boldsymbol{\Xi}_A \boldsymbol{\Xi}_A} \right) + \text{tr}\left( \boldsymbol{\mathcal{G}}_i'' \mathlarger{\Sigma}_{ {\textstyle\mathstrut} \boldsymbol{\Xi}_A \boldsymbol{\Xi}_A} \right)\text{tr}\left( \boldsymbol{\mathcal{G}}_j'' \mathlarger{\Sigma}_{ {\textstyle\mathstrut} \boldsymbol{\Xi}_A \boldsymbol{\Xi}_A} \right)
\end{equation}


\begin{equation}
    %
    \mathlarger{\Sigma}_{ {\textstyle\mathstrut} \boldsymbol{Z}_A \boldsymbol{Z}_A} = \begin{bmatrix}
        %
        \mathlarger{\Sigma}_{ {\textstyle\mathstrut} \boldsymbol{X}_A \boldsymbol{X}_A} & \mathlarger{\Sigma}_{ {\textstyle\mathstrut} \boldsymbol{X}_A \boldsymbol{Y}_A} \\
        %
        \mathlarger{\Sigma}_{ {\textstyle\mathstrut} \boldsymbol{Y}_A \boldsymbol{X}_A} & \mathlarger{\Sigma}_{ {\textstyle\mathstrut} \boldsymbol{Y}_A \boldsymbol{Y}_A}
        
    \end{bmatrix}
    %
\end{equation}


\begin{equation}
    \mathcal{I}\left(\boldsymbol{X}_A ; \boldsymbol{Y}_A  \right) = \frac{1}{2} \ln \left( \frac{| |}{| |} \right)
\end{equation}









==> Old/literature_review.tex <==
\subsection{Literature in Cislunar Operations:}

\textcolor{blue}{Notes from \cite{Davis_2017}: Orbit Maintenance and Navigation of Human Spacecraft at Cislunar Near Rectilinear Halo Orbits}



\subsection{Literature in the category SSAT:}

\subsection{Literature in the category information collection:}

\textcolor{blue}{Notes from \cite{Nakka_2022}: Information-Based Guidance and Control Architecture for Multi-Spacecraft On-Orbit Inspection}

\textbf{What was the purpose or motivation of this research or review?}

\begin{itemize}
    \item Presents a control architecture for an inspection spacecraft in stable Passive Relative Orbits (PROs). In this context, inspection is performed visually. 
\end{itemize}

\textbf{What data or methods are used?}

\begin{itemize}
    \item The authors use a framework that balances the information collection and control input of the inspector 
\end{itemize}


\textbf{What is the most important result obtained?}

\begin{itemize}
    \item The resulting trajectories jointly consider the observational coverage of the target spacecraft and the fuel/energy cost
\end{itemize}

\subsection{Literature in the category SCP:}

Notes from \cite{Oguri_2024}: \textbf{Chance-constrained control for safe spacecraft autonomy: convex programming approach}

\begin{itemize}
    \item Paper presents a robust path-planning framework for safe spacecraft autonomy under uncertainty 
    \item Develops a computationally tractable formulation based on convex programming 
    \item Rigorously formulates the safe autonomy problem, gathers and extends techniques in literature to accommodate key cost/constraint functions 
    \item Demonstrate on two cases -- orbit maintenance in cislunar space and orbit rendezvous -- under model uncertainty, execution error via Gates model
    \item Paper leverages recent advances in chance-constrained control and applies it the the spacecraft autonomy problem 
\end{itemize}

Notes from \cite{Acikmese_2007}: \textbf{Convex programming approach to powered descent and guidance for mars landing}

\begin{itemize}
    \item Convex programming algorithm for the numerical solution of the minimum fuel powered descent guidance problem -- \textcolor{red}{Notice how they use the term guidance here}
    \item Main contribution is a formulation of the trajectory optimization problem as a second order code programming problem 
    \item Direct numerical methods for trajectory optimization are attractive because explicit consideration of the necessary conditions (adjoint equations, transversality conditions, maximum principle) are not required -- \textcolor{red}{What are these again? I haven't thought about optimal control in so long...}
    \item Formulate as a second-order cone programming problem -- can be solved in Polynomial time 
    \item There exist interior point algorithms to solve these 
\end{itemize}

Notes from \cite{Mao_2017}: \textbf{Successive convexification of non-convex optimal control problems with state constraints}

\begin{itemize}
    \item The proposed algorithm successively convexifies the problem via a \textit{project-and-linearize} procedure
    \item Finding a global solution to a nonlinear programming problem is generally NP-hard
    \item Prior to successive convexification, there were SCP approaches. However, they did not have convergence gaurantees -- SCvx does!!
\end{itemize}


Notes from \cite{Gaias_2015}: \textbf{Impulsive Maneuvers for Formation Reconfiguration Using Relative Orbital Elements}

\begin{itemize}
    \item In contrast to the available literature, which focuses on case-by-case or problem specific solutions, this work seeks the systematic search and characterization of impulsive maneuvers of operational relevance 
\end{itemize}

Notes from \cite{Greaves_2023}: Autonomous Optical-Only Spacecraft-to-Spacecraft Absolute Tracking and Maneuver Classification in Cislunar Space

\begin{itemize}
    \item This paper demonstrates that relative optical measurements provide full inertial estimates of an agent and target spacecraft
    \item First, absolute tracking is tested for observability -- produces consistent filter results 
    \item The spacecraft-to-spacecraft absolute tracking method presents the opportunity to enhance the autonomy and robustness of tracking solutions 
\end{itemize}

==> first_order_analytic__gradient.tex <==
\subsubsection{Special Case for First-Order Covariance Approximation}

An analytical expression exists for the gradient of the form of mutual information derived in Section \ref{sec:MI_first_order_approximation}.  Starting with Eq. \ref{eqn:matrix_MI}, it can be written as
%
\begin{equation}
    \frac{\partial \mathcal{I}(\boldsymbol{X}_{\mathcal{A}}; \boldsymbol{Y}_{\mathcal{A}})}{\partial \boldsymbol{x}_{\mathcal{A}, \text{obs}_0}} = \frac{\partial}{\partial \boldsymbol{x}_{\mathcal{A}, \text{obs}_0}}\left[\frac{1}{2}\left(\ln|\Tilde{H}\Tilde{P}\Tilde{H}| - \ln|\Tilde{R}|  \right)\right].\label{eqn:MI_gradient}
\end{equation}


For a scalar value $\xi$, and some matrix $M$ that is a function of $\xi$, the matrix determinant derivative \cite{Petersen_2008} is
%
\begin{equation}
    \frac{d}{d \xi} \mathrm{det}(M(\xi)) = \mathrm{det}(M(\xi))\cdot \mathrm{tr}\left(M^{-1}(\xi) \frac{d}{d \xi} M(\xi)\right).
\end{equation}
%
Using this identity, the gradient in Eq.~\ref{eqn:MI_gradient} is 
%
\begin{equation}
    \frac{\partial \mathcal{I}(\boldsymbol{X}_{\mathcal{A}}; \boldsymbol{Y}_{\mathcal{A}})}{\partial \boldsymbol{x}_{\mathcal{A}, \text{obs}_0}}  = \frac{1}{2} \left[\sum_{j = 1}^m T_{j, j, 1}, \cdots, \sum_{j = 1}^m T_{j, j, 6N_s} \right],
\end{equation}
%
where $m$ here is the size of the square array $\Tilde{H}\Tilde{P}\Tilde{H}^\top$. The tensor array $T$ is
%
\begin{equation}
    T = \left(\Tilde{H}\Tilde{P}\Tilde{H}^{\top} + \Tilde{R}\right)^{-1}\times_1 \left[\frac{\partial \Tilde{H}}{\partial \boldsymbol{x}_{\mathcal{A}, obs_0}} \times_1 \Tilde{P} \Tilde{H}^\top + \Tilde{H} \Tilde{P} \times_1 \frac{\partial \Tilde{H}^\top}{\partial \boldsymbol{x}_{\mathcal{A}, \text{obs}_0}} \right].
\end{equation}
%
 The operation $B\times_n C$ denotes the mode-$n$ tensor/matrix product. Computation of the tensor $\frac{\partial \Tilde{H}}{\partial \boldsymbol{x}_{\mathcal{A}, \text{obs}_0}}$ is rather involved. Consider the second row, first column matrix block 
%
\begin{equation}
    \Tilde{H}^{2, 1} = H_{\mathcal{A}, 2}\Phi_{\mathcal{A}}(t_2, t_{\text{obs}_0}) = H_{\mathcal{A}, 2} \frac{\partial \boldsymbol{x}_{\mathcal{A}, 2}}{\partial \boldsymbol{x}_{\mathcal{A}, \text{obs}_0}}
\end{equation}
%
from Eq.~\ref{eqn:big_H} where, here, $t_1$ is replaced by $t_{\text{obs}_0}$ for consistency with this discussion. Then its corresponding partial derivative is
%
\begin{equation}
    \frac{\partial \Tilde{H}^{2, 1}}{\partial \boldsymbol{x}_{\mathcal{A}, \text{obs}_0}} = \left(\frac{\partial H_{\mathcal{A}, 2}}{\partial \boldsymbol{x}_{\mathcal{A}, 2}} \times_2 
    %
    \frac{\partial \boldsymbol{x}_{\mathcal{A}, 2}}{\partial \boldsymbol{x}_{\mathcal{A}, \text{obs}_0}}\right) \times_1 \frac{\partial \boldsymbol{x}_{\mathcal{A}, 2}}{\partial \boldsymbol{x}_{\mathcal{A}, \text{obs}_0}} +
    %
    H_{\mathcal{A}, 2} \times_1 \frac{\partial^2\boldsymbol{x}_{\mathcal{A}, 2}}{\partial \boldsymbol{x}_{\mathcal{A}, \text{obs}_0} \partial \boldsymbol{x}^\top_{\mathcal{A}, \text{obs}_0}}.
    %
\end{equation}

The matrix $\frac{\partial \boldsymbol{x}_{\mathcal{A}, 2}}{\partial \boldsymbol{x}_{\mathcal{A}, \text{obs}_0}}$ and tensor $\frac{\partial^2 \boldsymbol{x}_{\mathcal{A}, 2}}{\partial \boldsymbol{x}_{\mathcal{A}, \text{obs}_0} \partial \boldsymbol{x}^\top_{\mathcal{A}, \text{obs}_0}}$ are the first- and second-order state transition derivatives of the augmented state, respectively. A similar procedure can be repeated for all matrix blocks in Eq.~\ref{eqn:big_H} to form $\frac{\partial \Tilde{H}}{\partial \boldsymbol{x}_{\mathcal{A}, \text{obs}_0}}$.  


==> first_order_analytic_covariance.tex <==
The \textit{linearized} form of the joint covariance $\Sigma_{\tilde{\boldsymbol{Z}} \tilde{\boldsymbol{Z}}}$ is 
%
\begin{equation}
    \Sigma_{\tilde{\boldsymbol{Z}} \tilde{\boldsymbol{Z}} = \begin{bmatrix}
        \tilde{\mathcal{F}}\Sigma_{}\tilde{\mathcal{F}}^\top & \tilde{\mathcal{F}}\Sigma\tilde{\mathcal{H}}^\top\\
        
    \end{bmatrix}} 
\end{equation}


Under linear assumptions, the covariance in Eq. \ref{eqn:big_pz} can be expressed as


%
\begin{equation}
    \Tilde{\Sigma} = \begin{bmatrix}
        \Tilde{P} & \Tilde{\Gamma}\\
        \Tilde{\Gamma}^\top & \Tilde{S}
    \end{bmatrix} = 
    %
    \begin{bmatrix}
        \Tilde{\Phi}\Tilde{P}\Tilde{\Phi}^{\top} & \Tilde{\Phi} \Tilde{P} \Tilde{H}^{\top}\\
        %
        \Tilde{H}\Tilde{P}\Tilde{\Phi}^{\top} & \Tilde{H}\Tilde{P}\Tilde{H}^{\top} + \Tilde{R}
    \end{bmatrix}.
\end{equation}
%
The corresponding prior and conditional measurement densities are 
%
\begin{flalign}
    p\left(\boldsymbol{Y}_\mathcal{A}\right) &= \mathcal{N}\left(\boldsymbol{Y}_{\mathcal{A}}; \bar{\boldsymbol{Y}}_{\mathcal{A}}, \Tilde{S} \right) \label{eqn:predicted_augmented_measurement} \\
    &= \mathcal{N}\left(\boldsymbol{Y}_{\mathcal{A}}; \bar{\boldsymbol{Y}}_{\mathcal{A}}, \Tilde{H} \Tilde{P} \Tilde{H}^\top + \Tilde{R} \right),\nonumber
\end{flalign}
%
and
%
\begin{flalign}
    p\left(\boldsymbol{Y}_{\mathcal{A}}|\boldsymbol{X}_{\mathcal{A}}\right) &= \mathcal{N}\left(\boldsymbol{Y}_{\mathcal{A}}; \hat{\boldsymbol{Y}}_{\mathcal{A}}, \Tilde{S} - \Tilde{\Gamma}^{\top} \Tilde{P}^{-1} \Tilde{\Gamma} \right)\\
    %
    &= \mathcal{N}\left(\boldsymbol{Y}_{\mathcal{A}}; \hat{\boldsymbol{Y}}_{\mathcal{A}}, \Tilde{R} \right),\nonumber
\end{flalign}
%
respectively. Applying the form contained in the second line of Eq.~\ref{eqn:marginal_MI}, the mutual information between the stacked state vector and stacked measurement vector is 
%
\begin{equation}
   \begin{multlined}[b]
    \mathcal{I}(\boldsymbol{X}_{\mathcal{A}}; \boldsymbol{Y}_{\mathcal{A}}) = \mathbb{E}_{\boldsymbol{X}_{\mathcal{A}}}\left[\mathcal{D}_{\text{KL}}\left[p(\boldsymbol{Y}_{\mathcal{A}}|\boldsymbol{X}_{\mathcal{A}})\|p(\boldsymbol{Y}_{\mathcal{A}})\right]\right] =
    %
    \frac{1}{2} \ln\left( \frac{|\Tilde{H} \Tilde{P} \Tilde{H}^{\top} + \Tilde{R}|}{|\Tilde{R}|}\right).\label{eqn:matrix_MI}
    %
   \end{multlined}
\end{equation}
%
The block state error covariance matrix in Eq.~\ref{eqn:predicted_augmented_measurement} is defined as 
%
\begin{equation}
    \Tilde{P} = \text{blkdiag}\left(\left[P_{\mathcal{A}, 1}, Q_{\mathcal{A}, 1}, Q_{\mathcal{A}, 2} \cdots, Q_{\mathcal{A}, N_{\text{meas} - 1}} \right]\right),
\end{equation}
%
where the first block corresponds to the initial state error covariance of the sensor and targets: $ P_{\mathcal{A}, 1} = \text{blkdiag}\left(\left[P_{1}^1, P_{1}^{2},\cdots, P_{1}^{N_s}\right] \right)$. The subsequent diagonal blocks add the contributions attributed to the process noise: $Q_{\mathcal{A}, k} = \text{blkdiag}\left(\left[Q_k^1, Q_{k}^{2},\cdots, Q_{k}^{N_s} \right] \right)$. The block matrix providing partial derivatives of the stacked measurement with respect to the stacked state vector is defined as
%
\begin{equation}
    \Tilde{H} = \begin{bmatrix}
        H_{\mathcal{A}, 1} & \boldsymbol{0} & \boldsymbol{0} & \cdots & \boldsymbol{0}\\
        %
        H_{\mathcal{A}, 2} \Phi_{\mathcal{A}}(t_2, t_1) & H_{\mathcal{A}, 2} & \boldsymbol{0} & \cdots & \boldsymbol{0}\\
        %
        H_{\mathcal{A}, 3} \Phi_{\mathcal{A}}(t_3, t_1) & H_{\mathcal{A}, 3} \Phi_{\mathcal{A}}(t_3, t_2) & H_{\mathcal{A}, 3} &\cdots & \boldsymbol{0}\\
        %
        \vdots & \vdots & \vdots & \ddots & \vdots\\
        %
        H_{\mathcal{A}, N_{\text{meas}}}\Phi_{\mathcal{A}}(t_{N_{\text{meas}}}, t_1) & H_{\mathcal{A}, N_{\text{meas}}} \Phi_{\mathcal{A}}(t_{N_\text{meas}}, t_2) & H_{\mathcal{A}, N_{\text{meas}}} \Phi_{\mathcal{A}}(t_{N_\text{meas}}, t_3) & \cdots & H_{\mathcal{A}, N_{\text{meas}}}
    \end{bmatrix}\mbox{,}
    \label{eqn:big_H}
\end{equation}
%
where, assuming again the convention where the spacecraft indexed by $i = 1$ is the observer, 
%
\begin{equation}
    H_{\mathcal{A}, k} = \begin{bmatrix}
        %
        \frac{\partial \boldsymbol{y}_k^{2}}{\partial \boldsymbol{x}_{k}^1} & \frac{\partial \boldsymbol{y}_k^{2}}{\partial \boldsymbol{x}^{2}_{k}} & \boldsymbol{0} & \cdots & \boldsymbol{0}\\
        %
        \frac{\partial \boldsymbol{y}_k^{3}}{\partial \boldsymbol{x}^1_{k}} & \boldsymbol{0} & \frac{\partial \boldsymbol{y}_k^{3}}{\partial \boldsymbol{x}^{3}_{k}} &  \cdots & \boldsymbol{0}\\
        \vdots & \vdots & \vdots & \ddots & \vdots\\
        %
        \frac{\partial \boldsymbol{y}_k^{N_s}}{\partial \boldsymbol{x}^1_{k}} & \boldsymbol{0} & \boldsymbol{0} &  \cdots & \frac{\partial \boldsymbol{y}_k^{N_s}}{\partial \boldsymbol{x}^{N_s}_{k}}\\
        %
    \end{bmatrix},
\end{equation}
%
and
%
\begin{equation}
    \Phi_{\mathcal{A}}(t_k, t_\ell) = \text{blkdiag}\left(\left[\frac{\partial \boldsymbol{x}^1_{k}}{\partial \boldsymbol{x}^1_{ \ell}}, \cdots, \frac{\partial \boldsymbol{x}^{N_s}_{k}}{\partial \boldsymbol{x}^{N_s}_{ \ell}} \right] \right).
\end{equation}
%
Finally, the block measurement noise covariance
%
\begin{equation}
    \Tilde{R} = \text{blkdiag}\left(\left[R_{\mathcal{A}, 1}, R_{\mathcal{A}, 2}, \cdots, R_{\mathcal{A}, N_{\text{meas}}}\right]\right),
    \label{eqn:big_R}
\end{equation}
%
where $R_{{\mathcal{A}}, k} = \text{blkdiag}\left(\left[R, R, \cdots, R \right]\right)$, containing the measurement noise covariance for a single measurement, repeated $N_s - 1$ times.
